Turbulent transition in a channel with superhydrophobic walls: the effect of roughness anisotropy

Superhydrophobic surfaces dramatically reduce skin friction of overlying liquid flows. These surfaces are complex and numerical simulations usually rely on models for reducing this complexity. One of the simplest consists in finding an equivalent boundary condition through an homogenisation procedure, which in the case of channel flow over oriented riblets, leads to the presence of a small spanwise component in the homogenized base flow velocity. This work aims at investigating the influence of such a three-dimensionality of the base flow on stability and transition in a channel with walls covered by oriented riblets. Linear stability for this base flow is investigated: a new instability region, linked to cross-flow effects, is observed. Tollmien-Schlichting waves are also retrieved but the most unstable are three-dimensional. Transient growth is also affected as oblique streaks with non-zero streamwise wavenumber become the most amplified perturbations. When transition is induced by Tollmien-Schlichting waves, after an initial exponential growth regime, streaky structures with large spanwise wavenumber rapidly arise. Modal mechanisms appear to play a leading role in the development of these structures and a secondary stability analysis is realised to retrieve successfully some of their characteristics. The second scenario, initiated with crossflow vortices, displays a strong influence of nonlinearities. The flow develops into large quasi spanwise-invariant structures before breaking down to turbulence. Secondary stability on the saturated cross-flow vortices sheds light on this stage of transition. In both cases, cross-flow effects dominate the flow dynamics, suggestings the need to consider these effects when modelling superhydrophobic surfaces.

==> main2 <==
% This is jfm2esam.bib v1.0 08/14/02
%
@Book{Schmid,
  author = 	 "Schmid, P. \& Henningson, D.",
  title = 	 "Stability and Transition in Shear Flows",
  year = 	 "2001",
  publisher = "Springer"
}

@article{Uhlmann,
    author = "Uhlmann, M. \& Nagata, M.",
    title = "Linear stability of flow in an internally heated
rectangular duct",
    journal =      "J. Fluid Mech.",
    volume =       "551",
    pages =        "387-404",
    year =         "2006"
}

@article{Monokrousos,
    author = "Monokrousos, M. \textit{et. al}",
    title = "Nonequilibrium Thermodynamics and the Optimal Path to Turbulence in Shear Flows",
    journal =      "Phys. Rev. Lett.",
    volume =       "106",
    pages =        "134502",
    year =         "2010"
}

@article{Sameen,
    author = "Sameen, A. \& Govindarajan, R.",
    title = "The effect of wall heating on instability of channel flow",
    journal =      "J. Fluid. Mech.",
    volume =       "577",
    pages =        "417-442",
    year =         "2007"
}

@article{Biau,
    author = "Biau, D. \& Bottaro, A.",
    title = "The effect of stable thermal stratification on shear flow stability",
    journal =      "Phys. Fluids.",
    volume =       "16",
    number =       "12",
    year =         "2004"
}

@book{Trefethen,
    author = "Trefethen",
    title = "Spectral methods in MATLAB",
    year =         "2001",
    publisher = "SIAM"
}

@phdthesis{Jerome,
    author = "Jerome, J.J.S.",
    title = "Transient Growth in Rayleigh-Bénard-Poiseuille/Couette flows",
    school =       "Ecole Polytechnique",
    year =         "2011"
}

@article{Onsager,
    author = "Onsager, L.",
    title = "Reciprocal relations in irreversible processes. I",
    journal =      "Phys. Rev.",
    volume =       "37",
    number =       "405",
    year =         "1931"
}

@Book{Prigogine,
  author = 	 "Prigogine, I. \& Kondepudi D.",
  title = 	 "Modern Thermodynamics: From Heat Engines to Dissipative Structures",
  year = 	 "1998",
  publisher = "Wiley"
}

@article{Goody,
    author = "Goody, R.",
    title = "Maximum Entropy Production in Climate Theory",
    journal =      "J. Atmos. Sci.",
    volume =       "64",
    pages =        "2735–2739",
    year =         "2007"
}

@article{Schmid_b,
    author = "Schmid, P. \& Brandt, L.",
    title = "Analysis of fluid systems: stability, receptivity, sensitivity",
    journal =      "Appl. Mech. Rev.",
    volume =       "66",
    number =        "024803 ",
    year =         "2014"
}

@article{Nagata,
    author = "Nagata, M. \& Generalis, S.",
    title = "Transition in Convective Flows Heated Internally",
    journal =      "J. Heat Trans.",
    volume =       "124",
    number =        "635",
    year =         "2002"
}

@article{Generalis,
    author = "Generalis, S. \& Nagata, M.",
    title = "Transition in Homogeneously Heated Inclined Plane Parallel Shear Flows",
    journal =      "J. Heat Trans.",
    volume =       "125",
    number =        "795",
    year =         "2003"
}

@article{Kaminski,
    author = "Kaminski, A.K., Caulfield, C.P., Taylor J.R.",
    title = "Transient growth in strongly stratified
    shear layers",
    journal =      "J. Fluid Mech.",
    volume =       "758",
    pages =        "R4",
    year =         "2014"
}

@article{Coelho,
    author = "Coelho, P.M. \& Pinho, F.T.",
    title = "A generalized Brinkman number for non-Newtonian duct flows",
    journal =      "J. Non-Newton. Fluid",
    volume =       "156",
    pages =        "202-206",
    year =         "2009"
}

@article{Tso_a,
    author = "Tso, C.P. \& Mahulikar, T.P.",
    title = "The use of the Brinkman number for single phase forced convective heat transfer in microchannels",
    journal =      "Int. J. Heat Mass Transf.",
    volume =       "42",
    pages =        "1813-1833",
    year =         "1999"
}

@article{Tso_b,
    author = "Tso, C.P. \& Mahulikar, T.P.",
    title = "The role of the Brinkman number in analysing flow transitions in microchannels",
    journal =      "Int. J. Heat Mass Transf.",
    volume =       "42",
    pages =        "1813-1833",
    year =         "1999"
}

@article{Orszag,
    author = "Orszag, S.",
    title = "Accurate solution of the Orr–Sommerfeld equation",
    journal =      "J. Fluid Mech.",
    volume =       "50",
    pages =        "689-703",
    year =         "1971"
}

@article{Farrell,
    author = "Farrell, B.F. \& Ioannou, P.J.",
    title = "Transient Development of Perturbations in Stratified Shear Flow",
    journal =      "J. Atmos. Sci.",
    volume =       "50",
    number =       "14",    
    pages =        "2201-2214",
    year =         "1993"
}

@article{Prigogine_2,
    author = "Glansdorff, I. \& Prigogine, P.",
    title = "On a general evolution criterion in macroscopic physics",
    journal =      "Physica",
    volume =       "30",
    pages =        "351-374",
    year =         "1964"
}

@article{Rebhan,
    author = "Rebhan, E.",
    title = "Maximum entropy production far from equilibrium: The example of strong shock waves",
    journal =      "Phys. Rev. A",
    volume =       "42",
    number =       "781",
    year =         "1990"
}

@article{Juretic,
    author = "Juretić, D. \& Županović, P.",
    title = "Photosynthetic models with maximum entropy production in irreversible charge transfer steps",
    journal =      "Comput. Biol. Chem.",
    volume =       "27",
    number =       "6",
    pages =        "541-553",
    year =         "2003"
}

@article{Paltridge,
    author = "Paltridge, G.W.",
    title = "Climate and thermodynamic systems of maximum dissipation",
    journal =      "Nature",
    volume =       "279",
    pages =        "630-631",
    year =         "1979"
}

@article{Ozawa,
    author = "Ozawa, H. \& Ohmura, N.",
    title = "The second law of thermodynamics and the global climate system: a review of the maximum entropy production principle",
    journal =      "Rev. Geophys.",
    volume =       "41",
    number =       "4",
    year =         "2003"
}

@article{LeDizes,
    author = "Le Dizès, S.",
    title = "Modal growth and non-modal growth in a stretched shear layer",
    journal =      "Eur. J. Mech. B Fluids",
    volume =       "22",
    pages =       "411-430",
    year =         "2003"
}

@article{Alizard,
    author = "Alizard, F., Robinet, J.C.",
    title = "Transient growth in a right-angled streamwise corner",
    journal =      "Eur. J. Mech. B Fluids",
    volume =       "37",
    pages =       "99-111",
    year =         "2013"
}

@article{Ayala,
    author = "Ayala, D., Protas, B.",
    title = "On maximum enstrophy growth in a hydrodynamic system",
    journal =      "Physica D",
    volume =       "37",
    pages =       "1553-1563",
    year =         "2011"
}

@article{DiVita,
    author = "Di Vita, A.",
    title = "Maximum or minimum entropy production? How to select a necessary criterion of stability for a dissipative fluid or plasma",
    journal =      "Phys. Rev. E",
    volume =       "81",
    number =       "041137",
    year =         "2010"
}

@article{Brandt,
    author = "Brandt, L.",
    title = "The lift-up effect: The linear mechanism behind transition and turbulence in shear flows",
    journal =      "Eur. J. Mech. B Fluids",
    volume =       "47",
    pages =       "80-96",
    year =         "2014"
}

@article{Nourgaliev,
    author = "Nourgaliev, R. \& Dinh, T. ",
    title = "The investigation of turbulence characteristics in an internally-heated unstably-stratified fluid layer",
    journal =      "Nucl. Engng. Design",
    volume =       "178",
    pages =       "235-258",
    year =         "1997"
}

@article{Kikuchi,
    author = "Kikuchi, Y., Shioyama, T. ",
    title = "Turbulent heat transport in a horizontal fluid layer
    heated internally and from below",
    journal =      "Int. J. Heat Mass Transf.",
    volume =       "29",
    pages =       "451-461",
    year =         "1986"
}

@article{Tritton,
    author = "Tritton, D. ",
    title = "Internally heated convection in the atmosphere of Venus and in the laboratory",
    journal =      "Nature",
    volume =       "257",
    pages =       "110-112",
    year =         "1975"
}

@article{Tritton_b,
    author = "Tritton, D. \& Zarraga, M. ",
    title = "Convection in horizontal layers with internal heat generation: experiments",
    journal =      "J. Fluid Mech.",
    volume =       "30",
    pages =       "21-32",
    year =         "1967"
}

@article{Orr,
    author = "Orr, W.M.",
    title = "The stability or instability of the steady motions of a perfect liquid and of a viscous liquid.",
    journal =      "Proc. R. Irish Acad. A",
    volume =       "27",
    pages =       "9-68",
    year =         "1907"
}

@article{Ellingsen,
    author = "Ellingsen, T. \& Palm, E.",
    title = "Stability of linear flow.",
    journal =      "Phys. Fluids",
    volume =       "18",
    pages =       "487",
    year =         "1975"
}

@article{Reddy,
    author = "Reddy, S.C. \& Henningson, D.S.",
    title = "Energy growth in viscous channel flows.",
    journal =      "J. Fluid Mech.",
    volume =       "252",
    pages =       "209-238",
    year =         "1993"
}

@article{Gustavsson,
    author = "Gustavsson, L.H.",
    title = "Energy growth of three-dimensional disturbances in plane Poiseuille flow.",
    journal =      "J. Fluid Mech.",
    volume =       "224",
    pages =       "241-260",
    year =         "1991"
}

@Book{Pazy,
  author = 	 "Pazy, A. ",
  title = 	 "Semigroups of linear operators andapplication to partial differential equations.",
  year = 	 "1983",
  publisher = "Springer"
}

%% End of file `jfm2esam.bib'.

